Hierarchy Builder: Organizing Textual Spans into a Hierarchy to Facilitate Navigation

Information extraction systems often produce hundreds to thousands of strings on a specific topic. We present a method that facilitates better consumption of these strings, in an exploratory setting in which a user wants to both get a broad overview of what's available, and a chance to dive deeper on some aspects. The system works by grouping similar items together and arranging the remaining items into a hierarchical navigable DAG structure. We apply the method to medical information extraction.

==> figures/relationsTable.tex <==
\begin{table}[h]
    \centering
    \graphicspath{ {./figures/relationsTable.png}
    \caption{represents the relations among the input spans}
    \label{tab:relationsTable}
\end{table}
